On the Minimax Optimality of the EM Algorithm for Learning Two-Component Mixed Linear Regression

We study the convergence rates of the EM algorithm for learning two-component mixed linear regression under all regimes of signal-to-noise ratio (SNR). We resolve a long-standing question that many recent results have attempted to tackle: we completely characterize the convergence behavior of EM, and show that the EM algorithm achieves minimax optimal sample complexity under all SNR regimes. In particular, when the SNR is sufficiently large, the EM updates converge to the true parameter $\theta^{*}$ at the standard parametric convergence rate $\mathcal{O}((d/n)^{1/2})$ after $\mathcal{O}(\log(n/d))$ iterations. In the regime where the SNR is above $\mathcal{O}((d/n)^{1/4})$ and below some constant, the EM iterates converge to a $\mathcal{O}({\rm SNR}^{-1} (d/n)^{1/2})$ neighborhood of the true parameter, when the number of iterations is of the order $\mathcal{O}({\rm SNR}^{-2} \log(n/d))$. In the low SNR regime where the SNR is below $\mathcal{O}((d/n)^{1/4})$, we show that EM converges to a $\mathcal{O}((d/n)^{1/4})$ neighborhood of the true parameters, after $\mathcal{O}((n/d)^{1/2})$ iterations. Notably, these results are achieved under mild conditions of either random initialization or an efficiently computable local initialization. By providing tight convergence guarantees of the EM algorithm in middle-to-low SNR regimes, we fill the remaining gap in the literature, and significantly, reveal that in low SNR, EM changes rate, matching the $n^{-1/4}$ rate of the MLE, a behavior that previous work had been unable to show.

==> Arxiv_preliminary.tex <==

\section{Preliminaries}
\label{sec:experiments}
We first provide an overview for Gaussian mixture of experts and the convergence rates of MLE in Section~\ref{eq:Gaussian_mixture_expert}. Then, in Sections~\ref{sec:experiment_independent} and~\ref{sec:experiment_dependent}, we motivate our study with the behavior of EM algorithm via extensive experiments under weakly separated linear mixed regression and linear linear mixed-effect model, respectively specific instances of algebraic independent and dependent link functions in Gaussian mixture of experts.  
\subsection{Gaussian mixtures of expert and convergence rates of MLE}
\label{eq:Gaussian_mixture_expert}
We assume that $(X_{1},Y_{1}), \ldots, (X_{n}, Y_{n})$ are i.i.d.\ samples from finite Gaussian mixture of experts that admits the following density function:
\begin{align}
\label{eq:true_density}
    g_{\text{true}}(x, y) : = \parenth{\sum_{i = 1}^{k} \pi_{i}^{*}f(y|h_{1}(x,\theta_{i}^*), h_{2}^2(x,\sigma_{i}^*))} \bar{f}(x),
\end{align}
\genecomment{We need to specify the parameter space of the parameters.}
where $f(y| \eta, \tau)$ is univariate Gaussian distribution with location parameter $\eta$ and scale parameter $\tau$; $h_{1}(X,\theta)$ and $h_{2}(X,\sigma)$ respectively denote link functions associated with the location and scale parameters; $\bar{f}(x)$ is the given density function on $X$. In the paper, we assume that the mixing weights $\pi^{*}$ are independent of the covariates $X$. In general, the true parameters $(\pi_{i}^{*}, \theta_{i}^*, \sigma_{i}^{*})_{i = 1}^{k}$ are unknown and we estimate them from the data. In order to do that, we fit the data by a Gaussian mixture of experts with $k$ components of the following form
\begin{align}
    \label{eq:fit_density}
    g_{\text{fit}}(x, y) = \parenth{\sum_{i = 1}^{k} \pi_{i} f(y|h_{1}(x,\theta_{i}), h_{2}^2(x,\sigma_{i}))} \bar{f}(x).
\end{align}
In order to facilitate the presentation, we denote $T(\pi^{*}, \theta^{*}, \eta^{*}) : = \min_{1 \leq i \neq j \leq k} \enorm{\theta_{i}^{*} - \theta_{j}^{*}} + \enorm{\sigma_{i}^{*} - \sigma_{j}^{*}}$ as minimum separation among mixture parameters of the true model.  
\paragraph{MLE approach and its convergence:} A popular approach to estimate the parameters $(\pi_{i}, \theta_{i}, \eta_{i})_{i = 1}^{k}$ is maximum likelihood estimation (MLE). It is equivalent to estimate the probability measure $G = \sum_{i = 1}^{k} \pi_{i} \delta_{(\theta_{i}, \sigma_{i})}$. Then, the MLE is given by:
\begin{align}
    \label{eq:mle_def}
    \widehat{G}_{n} = \sum_{i = 1}^{k} \widehat{\pi}_{i} \delta_{(\widehat{\theta}_{i}, \widehat{\sigma}_{i})} \in \mathop{\arg \max}_{G} \frac{1}{n} \sum_{i = 1}^{n} \log (g_{\text{fit}}(X_{i}, Y_{i})).
\end{align}
The parametric convergence rates $n^{-1/2}$ of MLE under well-separated Gaussian mixtures of experts, namely, $T(\pi^{*}, \theta^{*}, \sigma^{*}) \geq c$ for some fixed positive constant $c$ independent of $n$, had been established in~\cite{Tanner-conf-1999, Tanner-1999, Tanner-Neural-1999}. However, for weakly separated settings of these models, namely, when $T(\pi^{*}, \theta^{*}, \sigma^{*})$ goes to 0 as the sample size goes to infinity, the convergence rates of MLE have remained poorly understood. Under the no separation setting, i.e., $T(\pi^{*}, \sigma^{*}, \eta^{*}) = 0$, Ho et al.~\cite{ho2019rate} introduced the notion of \emph{algebraic independence} between the expert functions to characterize the convergence rates of MLE. That notion entails that $\frac{\partial{h_{2}^2}}{\partial{\sigma}}(X, \sigma)$ and $\frac{\partial{h_{1}}}{\partial{\theta}}(X, \theta) \otimes \frac{\partial{h_{1}}}{\partial{\theta}}(X, \theta)$ are linear independent for almost surely $x$ where $u \otimes v$ denotes the outer product between vectors $u$ and $v$. Given that notion, under the no separation setting they demonstrated that
\begin{enumerate}
    \item When the expert functions $h_{1}$ and $h_{2}^2$ are algebraically independent, then $W_{2}(\widehat{G}_{n}, G_{*}) =  \mathcal{O}_{p}(n^{-1/4})$ where $G_{*} = \sum_{i = 1}^{k} \pi_{i}^{*} \delta_{(\theta_{i}^{*}, \sigma_{i}^{*})}$ denotes the true probability measure and $W_{2}$ is second order Wasserstein distance~\cite{Villani-03}. That result indicates that the convergence rates of MLE for estimating $\theta_{i}^{*}$ and $\sigma_{i}^{*}$ can be as slow as $n^{-1/4}$ while that of $\pi_{i}^{*}$ is $n^{-1/2}$ for all $i \in [k]$.
    \item When the expert function $h_{1}$ and $h_{2}^2$ are algebraically dependent, the convergence rates of MLE to the true parameters can be much slower than $n^{-1/4}$ and depend the partial differential equation (PDE) structures between the link functions (cf. Section 4 in~\cite{ho2019rate}). 
\end{enumerate}
\subsection{Algebraically independent setting - mixed linear regression with unknown variance noise} 
\label{sec:experiment_independent}
In this section, we investigate the behaviors of EM algorithm under the weakly separated settings of Gaussian mixture of experts when the link functions are algebraically independent. We particularly focus on the popular mixed linear regression \cite{de1989mixtures, viele2002modeling}, which is given by:
\begin{align}
\label{eq:true_density_mixed_linear}
    g_{\text{true}}(x, y) : = \parenth{\sum_{i = 1}^{k} \pi_{i}^{*}f(y| (\theta_{i}^*)^{\top} X, (\sigma_{i}^{*})^2)} \bar{f}(x).
\end{align}
It indicates that $h_{1}(X, \theta) = \theta^{\top} X$ and $h_{2}^2(X, \sigma) = \sigma^2$ for all $\theta$ and $\sigma$. It is clear that $h_{1}$ and $h_{2}^2$ are algebraically independent. We fit the data by using the model $g_{\text{fit}}(x, y) : = \parenth{\sum_{i = 1}^{k} \pi_{i}f(y| (\theta_{i})^{\top} X, \sigma_{i})} \bar{f}(x)$. For our experiments, we specifically consider the following settings with the parameters:
\begin{enumerate}
    \item \textbf{Setting (I.1) - High SNR regime}: $k = 2$, $\sigma_{1}^{*} = \sigma_{2}^{*}$, $\|\theta_{1}^{*} - \theta_{2}^{*}\| \geq C n^{-1/4}$ for some universal constant $C$. Furthermore, in the fitted model, $\sigma_{1} = \sigma_{2}$ and we use EM algorithm for $(\pi_{i}, \theta_{i})_{i=1}^{2}$. The performance of EM is summarized in Figure~\ref{}. \genecomment{We need to use Wasserstein distance to measure the performance.}  
    \item \textbf{Setting (I.2) - Low SNR regime}: We use similar setup as that of setting (I.2) except that $\|\theta_{1}^{*} - \theta_{2}^{*}\| \leq C n^{-1/4}$. Experiment in that setting is in Figure~\ref{}.
    \item \textbf{Setting (I.3) - Low SNR regime}: $k = 3$, $\max_{1 \leq i \neq j \leq 3} \|\theta_{i}^{*} - \theta_{j}^{*}\|^2 + |(\sigma_{i}^{*})^2 - (\sigma_{j}^{*})^2|  \leq C n^{-1/2}$. \jycomment{(i) Do we measure $n$ vs final statistical error? (ii) Do we report total number of iterations? (iii) What do we want to demonstrate with $k=3$? (iv) Is Wasserstein distance different from $l_2$-error (+ error in variance)?} \genecomment{(i) Yes; (ii) Yes, we would like to show it is at the order $\sqrt{n/d}$ for low SNR regime and $\log(n/d)$ for strong SNR regime;(iii) We want to show that the phenomenon with EM is beyond mixture of two and we use mixture of two in theory just for the simplication.}
\end{enumerate}
\subsection{Algebraically dependent setting - linear mixed-effect model}
\label{sec:experiment_dependent}
Moving to the algebraically dependent setting, we specifically consider the popular mixture of linear mixed-effect models \cite{verbeke1996linear}. The model admits the following form:
\begin{align}
\label{eq:true_density_mixed_effect}
    g_{\text{true}}(x, y) : = \parenth{\sum_{i = 1}^{k} \pi_{i}^{*}f(y| (\theta_{i}^*)^{\top} X, (\sigma_{i}^{*})^2 \|X\|^2)} \bar{f}(x).
\end{align}
It shows that we choose $h_{1}(X, \theta) = \theta^{\top} X$ and $h_{2}^2(X, \sigma) = \sigma^2 \|X\|^2$. We can check that the expert functions $h_{1}$ and $h_{2}^2$ are algebraically dependent when $d = 1$ while they are algebraically independent when $d \geq 2$. For our experiments, we consider the following settings:
\begin{enumerate}
    \item \textbf{Setting (D.1) - Low SNR regime}: $k = 2$, $\sigma_{1}^{*} = \sigma_{2}^{*}$. When $d = 1$, we set $\|\theta_{1}^{*} - \theta_{2}^{*}\| \leq C_{1} n^{-1/8}$ for some positive constant $C_{1}$. When $d \geq 2$, we choose $\|\theta_{1}^{*} - \theta_{2}^{*}\| \leq C_{2} n^{-1/4}$ where $C_{2}$ is some positive constant. In the fitted model, we choose $\sigma_{1} = \sigma_{2}$ and use EM algorithm to estimate the parameters. Experiments with the algorithm is in Figure~\ref{}.
    \item \textbf{Setting (D.2) - Low SNR regime}: $k = 3$. When $d = 1$, $\max_{1 \leq i \neq j \leq 3} |\theta_{i}^{*} - \theta_{j}^{*}|^4 + |(\sigma_{i}^{*})^2 - (\sigma_{j}^{*})^2|^2  \leq C_{1} n^{-1/2}$. When $d \geq 2$, $\max_{1 \leq i \neq j \leq 3} \|\theta_{i}^{*} - \theta_{j}^{*}\|^2 + |(\sigma_{i}^{*})^2 - (\sigma_{j}^{*})^2|  \leq C_{1} n^{-1/2}$. 
\end{enumerate} 
